Towards Robust Deep Learning with Ensemble Networks and Noisy Layers

In this paper we provide an approach for deep learning that protects against adversarial examples in image classification-type networks. The approach relies on two mechanisms:1) a mechanism that increases robustness at the expense of accuracy, and, 2) a mechanism that improves accuracy but does not always increase robustness. We show that an approach combining the two mechanisms can provide protection against adversarial examples while retaining accuracy. We formulate potential attacks on our approach with experimental results to demonstrate its effectiveness. We also provide a robustness guarantee for our approach along with an interpretation for the guarantee.

==> Plots/mnist_normal/Figure_adv2_freq.tex <==
\begin{figure} [t]
\centering
\begin{multicols}{2}
\begin{subfigure}{0.25\textwidth}
\caption{\label{fig:freq_changed_target_mnist} To Target }
\vspace {-.2cm}
\begin{tikzpicture}
\begin{axis}[
    xlabel={Perturbation},
    ylabel={Frequency},
   xlabel style={at={(0.4,1.5ex)}},
    ylabel style={at={(0.18,10ex)}},
    xmin=-0.015, xmax=0.5,
    ymin=-0.0005, ymax=0.0125,
    xtick={0.0, 0.1, 0.2,0.3,0.4,0.5},
    ytick={0.0, 0.002, 0.004, 0.006, 0.008},
    yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=3},
    scaled y ticks=false,
    mark size=1.0pt,
    ymajorgrids=true,
    grid style=dashed,
  %  x dir=reverse,
    legend style={font=\fontsize{5}{3}\selectfont},
    legend cell align={left},
    label style={font=\fontsize{7}{3}\selectfont},
    tick label style={font=\fontsize{4}{3}\selectfont},
    width=\textwidth,
    height=\textwidth,   
%    legend style={at={(1,0)},anchor=north west, font=\fontsize{5}{3}\selectfont},
     legend style={at={(0.32,1)},anchor=north, font=\fontsize{5}{3}\selectfont, style={row sep=0.01cm}},
%    legend style={anchor=north west, font=\fontsize{4}{3}\selectfont},
]
 
\addplot[
only marks,
    color=blue,
    mark=star,
    ]
file [skip first] {Plots/mnist_normal/Figure_adv2target_freq.png_1.txt};
    \legend{Noisy Adv. Inputs}
    
\addplot[
only marks,
    color=green,
    mark=o,
    style= {solid, fill=green},
    only marks,
    ]
file [skip first] {Plots/mnist_normal/Figure_adv2target_freq.png_0.txt};
    \addlegendentry{Adv. Inputs}    

\end{axis}
\end{tikzpicture}
\end{subfigure}
\columnbreak
\begin{subfigure}{0.25\textwidth}
\caption{\label{fig:freq_changed_other_mnist}To Others}
\vspace {-.2cm}
\begin{tikzpicture}
\begin{axis}[
    xlabel={Perturbation},
    ylabel={Frequency},
   xlabel style={at={(0.4,1.5ex)}},
    ylabel style={at={(0.18,10ex)}},
    xmin=-0.015, xmax=0.5,
    ymin=-.0005, ymax=0.0125,
    xtick={0.0, 0.1, 0.2,0.3,0.4,0.5},
    ytick={0.0, 0.002, 0.004, 0.006, 0.008},
    yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=3},
    scaled y ticks=false,
    mark size=1.0pt,
    ymajorgrids=true,
    grid style=dashed,
    legend style={font=\fontsize{5}{3}\selectfont},
    legend cell align={left},
    label style={font=\fontsize{7}{3}\selectfont},
    tick label style={font=\fontsize{4}{3}\selectfont},
    width=\textwidth,
    height=\textwidth,   
     legend style={at={(0.32,1)},anchor=north, font=\fontsize{5}{3}\selectfont, style={row sep=0.01cm}},
]
 
\addplot[
    color=blue,
    mark=star,
    only marks,
    ]
file [skip first] {Plots/mnist_normal/Figure_adv2other_freq.png_1.txt};
    \legend{Noisy Adv. Inputs}
    
\addplot[
    color=green,
    mark=o,
    style= {solid, fill=green},
    only marks,
    ]
file [skip first] {Plots/mnist_normal/Figure_adv2other_freq.png_0.txt};
    \addlegendentry{Adv. Inputs}
    
\end{axis}
\end{tikzpicture}
\end{subfigure}
\end{multicols}
\vspace {-.5cm}
%\begin{tikzpicture}
%{\footnotesize
%\begin{customlegend}[legend columns=-1,legend style={draw=none,column sep=1ex,font=\fontsize{7}{7}\selectfont},legend entries={Noisy Adv. Inputs, Adv. Inputs}]
%
%    \addlegendimage{blue,fill=blue!50!blue,mark=star, mark options={mark size=2pt,solid, line width=1pt}, only marks}
%    \addlegendimage{green,fill=green!50!green,mark=o, mark options={mark size=2pt,solid, line width=1pt}, only marks}
%    \end{customlegend}
%    }
%\end{tikzpicture}


\caption{\label{fig:aggregate_changed_mnist} MNIST Ensemble: Aggregate Outputs Changed}

\end{figure}


==> Plots/mnist_normal/Figure_adv2correct.tex <==
\begin{figure} [t]
\centering
\begin{multicols}{2}
\begin{subfigure}{0.25\textwidth}
\caption{\label{fig:avg_accuracy_mnist} Average accuracy vs. perturbation }
\vspace {-.2cm}
\begin{tikzpicture}
\begin{axis}[
    xlabel={Perturbation},
    ylabel={Average Accuracy},
   xlabel style={at={(0.4,1.5ex)}},
    ylabel style={at={(0.18,10ex)}},
    xmin=-0.015, xmax=0.5,
    ymin=-.05, ymax=1.5,
    xtick={0.0, 0.1, 0.2,0.3,0.4,0.5},
    ytick={0,0.2,0.4,0.6,0.8,1.0},
    mark size=0.5pt,
    ymajorgrids=true,
    grid style=dashed,
    legend style={font=\fontsize{5}{3}\selectfont},
    legend cell align={left},
    label style={font=\fontsize{7}{3}\selectfont},
    tick label style={font=\fontsize{4}{3}\selectfont},
    width=\textwidth,
    height=\textwidth,   
     legend style={at={(.42,1)},anchor=north, font=\fontsize{5}{3}\selectfont, style={row sep=0.01cm}},
]

\addplot[
%only marks,
    color=blue,
    mark=o,
 %   style= {solid, fill=green},
    ]
file [skip first] {Plots/mnist_normal/trans_avg_accuracy.png_1.txt};
    \legend{Noisy Adv. Inputs}
\addplot[
%only marks,
    color=green,
    mark=star,
    ]
file [skip first] {Plots/mnist_normal/trans_avg_accuracy.png_0.txt};
    \addlegendentry{Adv. Inputs}    
    


\end{axis}
\end{tikzpicture}
\end{subfigure}
\columnbreak
\begin{subfigure}{0.25\textwidth}
\caption{\label{fig:perturb_distribution_correct_mnist}Perturbation distribution of correct outputs}
\vspace {-.2cm}
\begin{tikzpicture}
\begin{axis}[
    xlabel={Perturbation},
    ylabel={Frequency},
   xlabel style={at={(0.4,1.5ex)}},
    ylabel style={at={(0.18,10ex)}},
    xmin=-0.015, xmax=0.5,
    ymin=-.003, ymax=.09,
    xtick={0.0, 0.1, 0.2,0.3,0.4,0.5},
    ytick={0,0, 0.01, 0.020,0.03,0.04,0.05,0.06,0.07},
%    yticklabel style={/pgf/number format/fixed},
    yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=2},
    scaled y ticks=false,
    mark size=1.0pt,
    ymajorgrids=true,
    grid style=dashed,
    legend style={font=\fontsize{5}{3}\selectfont},
    legend cell align={left},
    label style={font=\fontsize{7}{3}\selectfont},
    tick label style={font=\fontsize{4}{3}\selectfont},
    width=\textwidth,
    height=\textwidth,   
     legend style={at={(0.68,1)},anchor=north, font=\fontsize{5}{3}\selectfont, style={row sep=0.01cm}},
]
 
\addplot[
    color=blue,
    mark=star,
    only marks,
    ]
file [skip first] {Plots/mnist_normal/Figure_adv2correct_freq.png_1.txt};
    \legend{Noisy Adv. Inputs}
    
\addplot[
    color=green,
    mark=o,
    style= {solid, fill=green},
    only marks,
    ]
file [skip first] {Plots/mnist_normal/Figure_adv2correct_freq.png_0.txt};
    \addlegendentry{Adv. Inputs}
    
\end{axis}
\end{tikzpicture}
\end{subfigure}
\end{multicols}
\vspace {-.5cm}
\caption{\label{fig:perturbation_accuracy_mnistensemble} MNIST Ensemble: Perturbation \& Accuracy}

\end{figure}


==> Plots/mnist_normal/Figure_flip2_count.tex <==
\begin{figure} [t]
\centering
\begin{multicols}{2}
\begin{subfigure}{0.25\textwidth}
\caption{\label{fig:count_changed_target_mnist} To Target }
\vspace {-.2cm}
\begin{tikzpicture}
\begin{axis}[
    xlabel={Perturbation},
    ylabel={Count},
   xlabel style={at={(0.4,1.5ex)}},
    ylabel style={at={(0.18,10ex)}},
    xmin=-0.015, xmax=0.5,
    ymin=-.5, ymax=14,
    xtick={0.0, 0.1, 0.2,0.3,0.4,0.5},
    ytick={0,2,4,6,8,10,12},
    mark size=1.0pt,
    ymajorgrids=true,
    grid style=dashed,
    legend style={font=\fontsize{5}{3}\selectfont},
    legend cell align={left},
    label style={font=\fontsize{7}{3}\selectfont},
    tick label style={font=\fontsize{4}{3}\selectfont},
    width=\textwidth,
    height=\textwidth,   
     legend style={at={(0.32,1)},anchor=north, font=\fontsize{5}{3}\selectfont, style={row sep=0.01cm}},
]
 
\addplot[
only marks,
    color=blue,
    mark=star,
    ]
file [skip first] {Plots/mnist_normal/Figure_flip2target_count.png_1.txt};
    \legend{Noisy Adv. Inputs}
    
\addplot[
only marks,
    color=green,
    mark=o,
    style= {solid, fill=green},
    only marks,
    ]
file [skip first] {Plots/mnist_normal/Figure_flip2target_count.png_0.txt};
    \addlegendentry{Adv. Inputs}    

\end{axis}
\end{tikzpicture}
\end{subfigure}
\columnbreak
\begin{subfigure}{0.25\textwidth}
\caption{\label{fig:count_changed_other_mnist}To Others}
\vspace {-.2cm}
\begin{tikzpicture}
\begin{axis}[
    xlabel={Perturbation},
    ylabel={Count},
   xlabel style={at={(0.4,1.5ex)}},
    ylabel style={at={(0.18,10ex)}},
    xmin=-0.015, xmax=0.5,
    ymin=-3, ymax=60,
    xtick={0.0, 0.1, 0.2,0.3,0.4,0.5},
    ytick={0,10,20,30,40,50},
    mark size=1.0pt,
    ymajorgrids=true,
    grid style=dashed,
    legend style={font=\fontsize{5}{3}\selectfont},
    legend cell align={left},
    label style={font=\fontsize{7}{3}\selectfont},
    tick label style={font=\fontsize{4}{3}\selectfont},
    width=\textwidth,
    height=\textwidth,   
     legend style={at={(0.32,1)},anchor=north, font=\fontsize{5}{3}\selectfont, style={row sep=0.01cm}},
]
 
\addplot[
    color=blue,
    mark=star,
    only marks,
    ]
file [skip first] {Plots/mnist_normal/Figure_flip2other_count.png_1.txt};
    \legend{Noisy Adv. Inputs}
    
\addplot[
    color=green,
    mark=o,
    style= {solid, fill=green},
    only marks,
    ]
file [skip first] {Plots/mnist_normal/Figure_flip2other_count.png_0.txt};
    \addlegendentry{Adv. Inputs}
    
\end{axis}
\end{tikzpicture}
\end{subfigure}
\end{multicols}
\vspace {-.5cm}
\caption{\label{fig:counts_changed_mnist} MNIST: Counts of Networks Changed}

\end{figure}


==> Sections/Discussion.tex <==
\section{Discussion}
The goals of our work might appear somewhat contradictory. On one-hand, we are providing a mechanism that protects against adversarial examples, and it relies on the ground that transferability properties of adversarial examples between networks are not \emph{completely} known. On the other hand, we've shown how easy it is to craft an adversarial example using superimposition, that would result in an example that can fool not only the original networks from which the example was crafted, but can potentially fool other networks as well (that is, in the absence of a protection mechanism). We believe the key to finding an adversarial example that will truly resist all protection mechanisms, including our work here, is to understand the transferability properties of such examples across different networks. Based on our testing results, it appears transferability depends very much on the complexity of the classification task. The images in the CIFAR10 dataset have many more features than those in the MNIST dataset, while the CIFAR10 and MNIST networks were trained with similar model architectures, the MNIST networks are much more prone to transferability than the CIFAR10 networks. Also, we note that it takes a much smaller amount of perturbations to craft an adversarial example on a single CIFAR10 network than it does for an MNIST network, which could mean that on a CIFAR10 image there is a small subset of pixels which are most important to the model. When this small subset of pixels varies across different models, then it becomes very unlikely that an adversarial example crafted with one model would succeed on a different model; unless there is some model-independent small subset of pixels which are universally important to every model.\\

%\noindent
%\textbf{Threat Analysis}
%
%\noindent
%We note that most adversarial examples failed because they relied on integrity of the outputs at a layer (in this paper we focused on the logits due to nature of the Carlini-Wagner attacks). Therefore, in the presence of the noisy logit mechanism, an adversary might try to circumvent this obstacle by trying to infer the genuine outputs from the noisy outputs. Note that since the neural network is not necessarily a continuous function, an average of the noisy outputs, which are function values of a random distribution, is not necessarily equal to the genuine output of the average of perturbed inputs. However, we remark that it is valuable to perform detailed testing on how well an average of the outputs can function as approximation to the genuine output, though we also remark that attacks of this sort would require much more effort as the adversary might need to collect a large number of outputs based on the same input for each iteration required in crafting an attack.

We note that transferability of neural networks was studied by Papernot et al. \citep{papernot2016transferability}, where it was shown in the experiments that transferability from one neural network to another was as high as 38\% using the Fast Gradient Sign method \citep{goodfellow2014explaining}. In \citep{papernot2016transferability}, they did not consider an explicit algorithm for attacking an ensemble model. In our testing results in Tables~\ref{tab:accuracy_clean_vs_super2} and \ref{tab:classification_clean_vs_super2}, we showed that using a simple superimposition of two adversarial examples, the average accuracy on the MNIST networks was reduced from 96.80\% to 55.30\%, with ensemble accuracy of 66.30\%. When three adversarial examples were used, the average accuracy was reduced from 95.60\% to 24.69\%, with ensemble accuracy of 26.67\%, as shown in Tables \ref{tab:accuracy_clean_vs_super3} and \ref{tab:classification_clean_vs_super3}. Note that transferability rate is also dependent on the classification task, where we saw in the same tables %Table \ref{tab:accuracy_clean_vs_super2} and \ref{tab:accuracy_clean_vs_super3} 
that the same experiments performed on the CIFAR10 dataset showed a much lower transferability rate on similar superimposition attacks.

